Modeling and Measuring Graph Similarity: The Case for Centrality Distance

The study of the topological structure of complex networks has fascinated researchers for several decades, and today we have a fairly good understanding of the types and reoccurring characteristics of many different complex networks. However, surprisingly little is known today about models to compare complex graphs, and quantitatively measure their similarity. This paper proposes a natural similarity measure for complex networks: centrality distance, the difference between two graphs with respect to a given node centrality. Centrality distances allow to take into account the specific roles of the different nodes in the network, and have many interesting applications. As a case study, we consider the closeness centrality in more detail, and show that closeness centrality distance can be used to effectively distinguish between randomly generated and actual evolutionary paths of two dynamic social networks.

==> backup.tex <==
\section{Analysis}

\subsection{Weighted \mg and centralities}
\label{sec:weight-mg-centr}



\subsection{Centrality to Graph Edit Distance}

What is exactly the link between graph distance and centrality measures?
Cospectral graphs exist, co-central graph also, so I guess the 'way back'
algorithm ($t^{-1}$) is not that simple.
If we consider sensitive centralities, we might want to build a path of simple
edits?

\section{Graph Distances}\label{sec:graph-dist}

In order to measure the similarity between two graphs $G_1,G_2 \in \mathcal{G}$,
we need a concept of \emph{(graph) distance}. Intuitively, a graph distance $d(G_1,G_2)$ should
represent how similar two graphs are (more similar for smaller $d$).
\begin{definition}[Graph Distance]
 A graph distance $d$ is
a function $d\colon (G_1,G_2) \to \mathbb{R}^{+}$, with the following properties:
\begin{description}
\item[Separability] $d(G_1,G_2)=0 \Leftrightarrow G_1 = G_2$
\item[Symmetry] $d(G_1,G_2) = d(G_2,G_1)$
\item[Triangle Inequality] $\forall x,y,z \in V(G), d(x,y)\leq d(x,z)+d(z,y)$
\end{description}
\end{definition}

The canonical example is the \emph{Graph Edit Distance} (\GED). The distance
$d_{\GED}(G_1,G_2)$ is the minimal number of steps to
transform $G_1$ into $G_2$, where in each \emph{step} an edge or a vertex can be added
or deleted.

\gilles{ trouver definition formelle. Jai eu du mal a en
  trouver et je crois qu'il faut passer par un algo (de Dijkstra) -cf
  \cite{robles2004string} qui transforme les graphes en strings, et ensuite
  utiliser la string edit distance (ou Levenstein), bien definie elle.}\\

  \matthieu{Je pense qu'on peut la dŽfinir par induction, mais c'est
  pareil.
  \begin{eqnarray}
  d_{ED}(g,g)=&0&\forall g \in \cal{G}\\
  d_{ED}(V\cup \{v\},E)=&d_{ED}(V,E)+1,& \forall v \notin V\\
  d_{ED}(V,E\cup \{(v,w))=&d_{ED}(V,E)+1, &\forall v,w \in V^2, (v,w)\notin E
  \end{eqnarray}
}

Let \md~be a distance on  \G. Let $G=(V,E) \in \G$. For all node $i \in V$, we
denote $G-\{i\}$  the removal of node $i$ from the graph.
More precisely, $G-\{i\} = (V-\{i\}, E-\{(i,.)\}-\{(.,i)\})$. \gilles{ Ici on a
  toujours le probleme de nommer les sommets (ou de quel ordre on utilise pour
  en faire un vecteur de dim. $n$.)}


While vectors of vertex centralities are typically used to gain insights into the nature of a given graph,
we argue that it can also be used to compare graphs to each other. Intuitively,
two graphs with a similar centrality characteristic are more likely to originate from
a similar setting, e.g., are different snapshots of an evolving network (e.g., due to user
mobility). Indeed, as we will see, there exist interesting connections between
centralities and graph distances. As a simple example, it is easy to see that
the Graph Edit Distance between two graphs $G_1$ and $G_2$ equals the difference (i.e., \emph{distance}) of the
degree centralities, $d_{\GED}(G_1,G_2) = |\sum_{v\in V(G_1)} c_{\DC}(v)$ $- \sum_{v\in V(G_2)} c_{\DC}(v)|$.

\subsection{Centrality Distance}

We propose to define graph distances based on centralities.
FIXME: intro graph of graph here??
\begin{definition}[Centrality (Graph) Distance]
Given a centrality $c$, we define the following \emph{Centrality Graph Distance} (\CGD)
$d_c$:
$$
d_c(G_1,G_2) = \sum_{v\in V(G_1)}
$$
\noindent for two neighboring graphs (FIXME). If not neighboring... distance
\end{definition}


  \begin{eqnarray*}
    t_\md: (V\times \G) & \rightarrow&\mathbb{R^+} \\
    (i, G)&  \mapsto&  \md(G,G-\{i\})
  \end{eqnarray*}
 It is important to notice that we do here define a centrality (because
 centrality has no other requirement than being a positive node-level
 measure). We refer hereafter to this centrality as the centrality
 \emph{induced} by \md.


Consider now the graph edit distance $d_{ED}$. Given $G$ and $i\in V$, the
minimum number of edit operations to go from $G-\{i\}$ to $G$ is:
\begin{itemize}
\item add node $i$
\item for each $j$ such that $(i,j) \in V_i$ ($V_i$ is defined with regards to $G$), add the corresponding edge
\end{itemize}
which costs $\vert V_i \vert +1 $ operations. Simple observation shows that $t_{ED}(i,G)
= c_d(i) +1$. We consider this as a very intriguing connection between the most
intuitive centrality on one side and the only known graph distance\footnote{to our knowledge} on the other.

STEFAN HERE I AM

\subsection{Defining centralities as induced graph distances}
\label{sec:defin-centr-as}

Following the previously mentioned relation between centrality and graph
distances, we know take a closer look at the properties an induced centrality
inherits from the graph distance application.

Firstly, because of the separability property, no node has a null induced
centrality. Secondly, any operation on the graph (adding/deleting an edge/vertex)
changes at least the induced centrality of a node. More formally, let \emph{sensitivity}
be the property of a centrality to react to any graph update:
\begin{definition}[Sensitive centrality]
  Let $c$ be a centrality. $c$ is sensitive if, for any graph $G(V,E)$, for
  any update $G'(V',E')$ of $G$, at least one centrality changes:
$$
\exists i \in V, c_{G}(i) \neq c_{G'}(i)
$$
\end{definition}

We show easily that any induced centrality is edge-sensitive: Let $d$ be a graph
distance, and $t_d$ the corresponding induced centrality. By contradiction,
assume $c$ is not sensitive. Then there exists a graph $G$ and an edge $\{i,j\}$
such that $\forall a \in V, t_d(a,G)=t_d(a,G \cup \{i,j\})$. In particular, we
have $t_d(i,G)=t_d(i,G \cup \{i,j\})$. Thus, $d(G,G-\{i\})=d(G \cup \{i,j\}
,(G\cup \{i,j\})-\{i\} )$. Since we have $G\cup \{i,j\}-\{i\}=G-\{i\}$ we thus
conclude $d(G,G-\{i\})=d(G \cup \{i,j\} ,G-\{i\})$. \gilles{OOps ca ne va pas
  suffire - il me semble meme que a pourrait etre faux}\matthieu{oui le passage
  avec "thus" me semble un peu ambitieux :-)}


\subsection{Introducing the Metagraph}
\label{sec:intr-metagr}

Let us now introduce the Metagraph, or graph of graphs.
\newcommand{\mg}{\ensuremath{\mathcal{MG}}~}
\newcommand{\mgk}{\ensuremath{\mathcal{MG}_k}~}
\begin{definition}
  The Metagraph \mg is the graph $G=(V,E)$ such that $V=\mathcal{G}$ and
  $E=\{\{i,j\}, d_{ED}(i,j)=1\}$.
\end{definition}

Any binary graph is a vertex in \mg and any serializable sequence of updates of
a graph defines a path in \mg.  Although \mg is infinite, it is possible to
observe some of its properties by partitioning it according to the number of
vertices of the graphs represented by its vertices:

\begin{definition}
  Let \mgk be the subgraph $(V_k,E_k)\subset \mg$ such that
  $$V_k=\{G\in  \mathcal{G}, \vert G \vert =k\}$$
  $$E_k=\{\{i,j\}, d_{ED}(i,j)=1\}$$.
\end{definition}

We have $\vert \mgk \vert= 2^{k\choose 2}$. Let $c(k,\ell)$ be the number of
edges of \mg between $\mathcal{MG}_k$ and $\mathcal{MG}_\ell$. It is easy to
observe that $\vert k - \ell\vert >1 \Rightarrow c(k,l)=0$. Moreover,
$c(k,k+1)=2^{k\choose 2}$ since it is always possible to add one vertex to a
graph of $k$ nodes. Interestingly, all the evolutions in $\mathcal{MG}_k$ that
leave such a single vertex unconnected are already described in
$\mathcal{MG}_{k-1}$, we thus conclude that from a pure ``structure'' point of
view, $\mathcal{MG}_{k-1} \subset \mathcal{MG}_{k}$.

\begin{lemma}
  $\mgk$ is bipartite
\end{lemma}

%\begin{proof}
  Let $G=(V,E)$ be a vertex of $\mathcal{MG}_{k}$. We have $\vert V \vert =
  k$. Let $\vert E \vert =m$. Since we are in \mgk, the only possible update
  operations are adding an edge or removing an edge. Let $V_e$ and $V_o$ be the
  subsets of \mgk that contains only even ($m\cong 0 (mod 2)$) and odd edge
  count graphs. Let $L$ be a cycle in \mgk. Since $L$ is a cycle, the start and
  end graph are identical, in particular the number of edges of the graph $m$ is
  conserved. Let $p$ the number of edge additions in the cycle, there has to be
  as many edge deletions to conserve $m$: the length of the cycle is $2p$ (since
  $m+p-p=m$). In other words, there is no odd-cycle in \mgk. \gilles{could be
    shorter...}
% Let $G_1$ and $G_2$ be two graphs of \mgk have respectively
%   $m_1$ and $m_2$ edges. Let $P$ be a path in \mgk from $G_1$ to $G_2$.
%\end{proof}

\gilles{ Du coup \mg est un graph parfait... Il est aussi bipartite par rapport
  aux sommets, mais je ne sais pas si c'est interessant de le noter}

\gilles{ Note the superexponential growth of \mgk : $\vert \mathcal{MG}_{5}
  \vert =1024 ; \vert \mathcal{MG}_{7} \vert > 2.10^6 ; \vert \mathcal{MG}_{9}
  \vert > 68.10^9$}


\gilles{ Truc cool, \mg est planaire ssi c'est un mineur (ou une subdivision) de
  $K_{3,3}$ le graphe bipartite complet de 6 sommets... faut que j'y rŽflechisse
mais c'est une direction cool ! }

\matthieu{j'ai pas compris la dernire remarque}

